Large-Scale Galaxy Bias

This review presents a comprehensive overview of galaxy bias, that is, the statistical relation between the distribution of galaxies and matter. We focus on large scales where cosmic density fields are quasi-linear. On these scales, the clustering of galaxies can be described by a perturbative bias expansion, and the complicated physics of galaxy formation is absorbed by a finite set of coefficients of the expansion, called bias parameters. The review begins with a detailed derivation of this very important result, which forms the basis of the rigorous perturbative description of galaxy clustering, under the assumptions of General Relativity and Gaussian, adiabatic initial conditions. Key components of the bias expansion are all leading local gravitational observables, which include the matter density but also tidal fields and their time derivatives. We hence expand the definition of local bias to encompass all these contributions. This derivation is followed by a presentation of the peak-background split in its general form, which elucidates the physical meaning of the bias parameters, and a detailed description of the connection between bias parameters and galaxy statistics. We then review the excursion-set formalism and peak theory which provide predictions for the values of the bias parameters. In the remainder of the review, we consider the generalizations of galaxy bias required in the presence of various types of cosmological physics that go beyond pressureless matter with adiabatic, Gaussian initial conditions: primordial non-Gaussianity, massive neutrinos, baryon-CDM isocurvature perturbations, dark energy, and modified gravity. Finally, we discuss how the description of galaxy bias in the galaxies' rest frame is related to clustering statistics measured from the observed angular positions and redshifts in actual galaxy catalogs.

==> xstring.tex <==
%  __________________________________________________
% |                                                  |
% |                                                  |
% |                  xstring v1.5a                   |
% |                                                  |
% |                  March 13 2009                   |
% |                                                  |
% |__________________________________________________|
%
% This is xtring.tex
%
% "xstring" package consists of the 11 following files:
%   xstring.tex (this file)
%   xstring.sty
%   README
%   xstring_doc_fr.tex, xstring_doc_fr.pdf (manual in french)
%   xstring_doc_en.tex, xstring_doc_en.pdf (manual in english)
%   test_latex.tex, test_latex.pdf (test file with LaTeX)
%   test_etex.tex, test_etex.pdf (test file with Plain eTeX)
%
% Christian Tellechea 2009
% email : unbonpetit@gmail.com
% -------------------------------------------------------------------
% This work may be distributed and/or modified under the
% conditions of the LaTeX Project Public License, either version 1.3
% of this license or (at your option) any later version.
% The latest version of this license is in
%
%     http://www.latex-project.org/lppl.txt
%
% and version 1.3 or later is part of all distributions of LaTeX
% version 2005/12/01 or later.
% -------------------------------------------------------------------
% This work has the LPPL maintenance status `maintained'.
%
% The Current Maintainer of this work is Christian Tellechea
% -------------------------------------------------------------------
\def\xstringversion     {1.5b}
\def\xstringdate        {2009/03/13}
\def\xstringfrenchdate  {13 mars 2009}
\def\xstringenglishdate {March $13^{\mathrm{th}}$ 2009}
\edef\CurrentAtCatcode  {\the\catcode`\@}
\catcode`\@=11
\newwrite\@xs@message% canal pour les messages
\newcount\integerpart\newcount\decimalpart% compteurs utilis\'es par xstring
\newif\if@xs@empty

\expandafter\ifx\csname @latexerr\endcsname\relax% on n'utilise pas LaTeX ?
	\immediate\write\m@ne{Package: xstring \xstringdate\space\space v\xstringversion\space\space String manipulations (C Tellechea)}%
	\long\def\@firstoftwo#1#2{#1}
	\long\def\@secondoftwo#1#2{#2}
	\long\def\@gobble#1{}
	\long\def\@ifnextchar#1#2#3{%
		\let\reserved@d=#1%
		\def\reserved@a{#2}%
		\def\reserved@b{#3}%
		\futurelet\@let@arg\@ifnch}
	\def\@ifnch{%
		\ifx\@let@arg\@sptoken
			\let\reserved@c\@xifnch
		\else
			\ifx\@let@arg\reserved@d
				\let\reserved@c\reserved@a
			\else
				\let\reserved@c\reserved@b
			\fi
		\fi
		\reserved@c}
	\def\:{\let\@sptoken= } \:
	\def\:{\@xifnch} \expandafter\def\: {\futurelet\@let@arg\@ifnch}
	\def\@ifstar#1{\@ifnextchar *{\@firstoftwo{#1}}}
	\long\def\@testopt#1#2{\@ifnextchar[{#1}{#1[{#2}]}}
	\def\@empty{}
\fi% fin des d\'efinitions LaTeX

\def\@xs@testempty#1{%
	\expandafter\ifx\expandafter\@empty\detokenize{#1}\@empty\@xs@emptytrue\else\@xs@emptyfalse\fi}

% Ouvre un groupe o\`u les catcodes sont \`a 12 et \`a 10 pour les espaces
% ensuite, appelle \@xs@ReadVerb qui lit un argument entre d\'elimiteurs verb
\def\@xs@MakeVerb{% lit 1 argument et le transforme en verb
	\begingroup% groupe o\`u les catcodes sont \`a 12 pour la lecture suivante
		\def\do##1{\catcode`##112\relax}%
		\dospecials% on entre dans le mode verb
		\obeyspaces% et on tient compte des espaces
		\@xs@ReadVerb}% et on va lire l'argument

% D\'efinit \@xs@ReadVerb qui lit un argument entre d\'elimiteurs verb
\def\setverbdelim#1{% d\'efinit quel est le d\'elimiteur de verb
	\expandafter\@xs@testempty\expandafter{\@gobble#1}%
	\if@xs@empty
	\else
		\begingroup
			\newlinechar`\^^J%
			\immediate\write\@xs@message
			{Package xstring Warning: verb delimiter is not a single token on input line \the\inputlineno^^J}%
		\endgroup
	\fi
	\def\@xs@ReadVerb##1#1##2#1{% lit ##2 qui est entre les d\'elimiteurs de verb
		\endgroup% on ferme le groupe
		\@xs@afterreadverb{##2}}}% on appelle l'ex\'ecution de fin

% Assigne l'argument entre d\'elimiteur verb dans la sc #1' +
\def\verbtocs#1{%
	\def\@xs@afterreadverb##1{\def#1{##1}}%
	\@xs@MakeVerb}

% Cette macro d\'eveloppe \'eventuellement #2
% puis le transforme en token et l'assigne \`a #1
\begingroup% on ouvre un groupe o\`u...
\catcode\z@12\relax% ...le caract\`ere 0 a 12 pour catcode
\gdef\tokenize#1#2{%
	\begingroup
		\@xs@def\@xs@reserved@A{#2}% on d\'eveloppe en accord avec \fullexpandarg ou \noexpandarg
		\def\@xs@AssignResult^^00##1^^00\@xs@nil{\gdef#1{##1}}% on assigne en tenant compte du \@xs@nil qui vient de la fin du fichier virtuel
		\everyeof{\@xs@nil}% met un \@xs@nil \`a la fin du fichier virtuel
		\endlinechar\m@ne
		\catcode\z@12\relax
		\expandafter\@xs@AssignResult\scantokens\expandafter{\expandafter^^00\@xs@reserved@A^^00}% on fait l'assignation
	\endgroup}%
\endgroup

% Macro tr\`es simple qui assigne ou affiche le r\'esultat, selon la pr\'esence
% ou non de #2 qui est l'argument optionnel venant en derni\`ere position des macros
\def\@xs@ReturnResult#1#2{%
	\def\@xs@argument@A{#1}%
	\@xs@testempty{#2}%
	\if@xs@empty
		\@xs@argument@A
	\else
		\let#2\@xs@argument@A
	\fi}

% Pas d'expansion des arguments
\def\normalexpandarg{%
	\let\@xs@def\def% on d\'efinit \@xs@call avec \def
	\def\@xs@expand##1{\unexpanded\expandafter{##1}}}
\let\noexpandarg\normalexpandarg% synonyme

% 1-d\'eveloppement du premier token des arguments
\def\expandarg{%
	\let\@xs@def\def% on d\'efinit \@xs@call avec \def
	\def\@xs@expand##1{\unexpanded\expandafter\expandafter\expandafter{##1}}}

% D\'eveloppement maximum des arguments
\def\fullexpandarg{%
	\let\@xs@def\edef% on d\'efinit\@xs@call avec \edef
	\def\@xs@expand##1{##1}}% et on neutralise \@xs@expand

\def\saveexpandmode{\let\@xs@saved@def\@xs@defarg\let\@xs@saved@expand\@xs@expand}
\def\restoreexpandmode{\let\@xs@defarg\@xs@saved@def\let\@xs@expand\@xs@saved@expand}

% Macro interne renvoyant #2 si son argument commence par une accolade ouvrante "{"
% et #3 sinon (Ulrich Diez sur comp.text.tex)
\def\@xs@ifbeginwithbrace#1{%
	\csname @%
		\expandafter\@gobble\string{% ne sert à rien si ce n'est \'equilibrer les accolades dans la d\'efinition
		\expandafter\@gobble\expandafter{\expandafter{\string#1}%
		\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\@firstoftwo
		\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\@gobble
		\expandafter\expandafter\expandafter\@gobble
		\expandafter\expandafter\expandafter{\expandafter\string\expandafter}\string}%
		\expandafter\@gobble\string}%
		\@secondoftwo{first}{second}oftwo%
	\endcsname}

% Cette macro interne prend la 1ere unit\'e syntaxique de #1 et assigne le r\'esultat \`a #2
\def\@xs@returnfirstsyntaxunit#1#2{%
	\def\@xs@groupfound{\expandafter\def\expandafter#2\expandafter{\expandafter{#2}}\@xs@gobbleall}% on met #2 dans des accolades et on finit
	\def\@xs@assignfirsttok##1##2\@xs@nil{\let\@xs@toks0\def#2{##1}}%
	\def\@xs@testfirsttok{%
		\let\@xs@next\@xs@assignfirsttok
		\ifx\@xs@toks\bgroup
			\expandafter\@xs@ifbeginwithbrace\expandafter{\@xs@argument}{\def\@xs@next{\afterassignment\@xs@groupfound\def#2}}{}%
		\fi
		\@xs@next}%
	\def\@xs@argument{#1}%
	\expandafter\@xs@testempty\expandafter{\@xs@beforespace#1 \@xs@nil}%
	\if@xs@empty
		\def\@xs@next{\expandafter\ifx\expandafter\@empty\detokenize\expandafter{\@xs@argument}\@empty\let#2\@empty\else\def#2{ }\fi}%
	\else
		\def\@xs@next{\expandafter\futurelet\expandafter\@xs@toks\expandafter\@xs@testfirsttok\@xs@argument\@xs@nil}%
	\fi
	\@xs@next}

% Cette macro interne enl\`eve la 1ere unit\'e syntaxique de #1 et assigne le r\'esultat \`a #2
\def\@xs@removefirstsyntaxunit#1#2{%
	\expandafter\@xs@testempty\expandafter{\@xs@beforespace#1 \@xs@nil}%
	\def\@xs@argument{#1}%
	\if@xs@empty
		\expandafter\@xs@testempty\expandafter{\@xs@argument}%
		\if@xs@empty
			\let#2\@empty
		\else
			\expandafter\expandafter\expandafter\def\expandafter\expandafter\expandafter#2%
			\expandafter\expandafter\expandafter{\expandafter\@xs@behindspace\@xs@argument\@xs@nil}%
		\fi
	\else
		\expandafter\expandafter\expandafter\def\expandafter\expandafter\expandafter#2%
		\expandafter\expandafter\expandafter{\expandafter\@gobble\@xs@argument}%
	\fi}

% Macros \`a arguments d\'elimit\'es pour les macros ci dessus
\def\@xs@beforespace#1 #2\@xs@nil{#1}
\def\@xs@behindspace#1 #2\@xs@nil{#2}
\def\@xs@returnfirstsyntaxunit@ii#1#2\@xs@nil{#1}
\def\@xs@gobbleall#1\@xs@nil{}

% Cette macro interne est utilis\'ee dans les macros \'etoil\'ees pour :
% 1) d\'evelopper l'argument selon qu'on a choisit \fullexpandarg
%    ou \normalexpandarg, et ceci \`a l'aide de la macro \@xs@def
% 2) Ensuite, on d\'etokenize ce d\'eveloppement de façon n'avoir plus que
%    des catcodes de 10 pour les espaces et 12 pour le reste.
\def\@xs@expand@and@detokenize#1#2{%
	\def#1{#2}%
	\expandafter\edef\expandafter#1\expandafter{\@xs@expand#1}% on d\'eveloppe #2 selon le mode de d\'eveloppement
	\edef#1{\detokenize\expandafter{#1}}}% puis on d\'etokenize et on assigne \`a #1

\def\@xs@expand@and@assign#1#2{\@xs@def#1{#2}}% on d\'eveloppe #2 selon \fullexpandarg ou \normalexpandarg

\def\@xs@edefaddtomacro#1#2{\edef#1{\unexpanded\expandafter{#1}#2}}
\def\@xs@addtomacro#1#2{\expandafter\def\expandafter#1\expandafter{#1#2}}

\def\@xs@argstring{0########1########2########3########4########5########6########7########8########9}
% \@xs@DefArg{3} met dans la sc \@xs@myarg les tokens "####1####2####3"
\def\@xs@DefArg#1{\def\@xs@defarg0##1#1##2\@xs@nil{\def\@xs@myarg{##1#1}}\expandafter\@xs@defarg\@xs@argstring\@xs@nil}
% \@xs@DefArg@{3} met dans la sc \@xs@myarg les tokens "[####1]####2####3####4"
\def\@xs@DefArg@#1{\expandafter\@xs@defarg@\expandafter{\number\numexpr#1+1}}
\def\@xs@defarg@#1{\def\@xs@defarg0##11##2#1##3\@xs@nil{\def\@xs@myarg{[##11]##2#1}}\expandafter\@xs@defarg\@xs@argstring\@xs@nil}
% \@xs@OneArg{3} met dans la sc \@xs@myarg les tokens "####3"
\def\@xs@OneArg#1{\expandafter\@xs@onearg\expandafter{\number\numexpr#1-1}{#1}}
\def\@xs@onearg#1#2{\def\@xs@defarg##1#1##2#2##3\@xs@nil{\def\@xs@myarg{##2#2}}\expandafter\@xs@defarg\@xs@argstring\@xs@nil}

% #1 : num\'ero du 1er argument; #2 : nombre de lignes; #3 argument optionnel; #4 : dernier num\'ero de l'argument devant être d\'etokenis\'e si \'etoile
\def\@xs@BuildLines#1#2#3#4{%
	\let\@xs@newlines\@empty
	\let\@xs@newargs\@empty
	\def\@xs@buildlines##1{%
		\expandafter\@xs@OneArg\expandafter{\number\numexpr##1+#1-1}%
		\edef\@xs@reserved@B{\noexpand\@xs@expand\csname @xs@arg@\romannumeral\numexpr##1\endcsname}%
		\ifnum##1=\@ne% si c'est le premier argument
			\@xs@testempty{#3}%
			\if@xs@empty
				\expandafter\@xs@addtomacro\expandafter\@xs@newargs\expandafter{\expandafter{\@xs@reserved@B}}%
				\edef\@xs@reserved@B{\ifnum##1>#4 @xs@def\else @xs@assign\fi}%
			\else% et s'il y a un argument optionnel alors, on met des crochets
				\expandafter\@xs@addtomacro\expandafter\@xs@newargs\expandafter{\expandafter[\@xs@reserved@B]}%
				\def\@xs@reserved@B{@xs@def}% ne pas d\'etok\'eniser l'argument optionnel grace au \@xs@def
			\fi
		\else
			\expandafter\@xs@addtomacro\expandafter\@xs@newargs\expandafter{\expandafter{\@xs@reserved@B}}%
			\edef\@xs@reserved@B{\ifnum##1>#4 @xs@def\else @xs@assign\fi}%
		\fi
		\edef\@xs@newlines{\unexpanded\expandafter{\@xs@newlines}\expandafter\noexpand\csname\@xs@reserved@B\endcsname\expandafter\noexpand\csname @xs@arg@\romannumeral\numexpr##1\endcsname{\@xs@myarg}}%
		\ifnum##1<#2\relax
			\def\@xs@next{\expandafter\@xs@buildlines\expandafter{\number\numexpr##1+1}}%
			\expandafter\@xs@next
		\fi}%
	\@xs@buildlines\@ne}

\def\@xs@newmacro{\@ifstar{\let\@xs@reserved@D\@empty\@xs@newmacro@}{\let\@xs@reserved@D\relax\@xs@newmacro@0}}
% #1 : dernier num\'ero de l'argument devant être d\'etokenis\'e
% #2 : nom de la macro publique
% #3 : argument optionnel (vide si pas d'arg optionnel)
% #4 : nombre d'arguments obligatoires
% #5 : utilisation de testopt (1 si oui, 0 si non)
% #6 : code de la macro
\def\@xs@newmacro@#1#2#3#4#5{%
	\edef\@xs@reserved@A{@xs@\expandafter\@gobble\string#2}%
	\edef\@xs@reserved@C{\expandafter\noexpand\csname\@xs@reserved@A @\ifx\@empty#3\@empty @\fi\endcsname}%
	\edef\@xs@reserved@B{%
		\ifx\@empty\@xs@reserved@D
			\def\noexpand#2{\noexpand\@ifstar
				{\let\noexpand\@xs@assign\noexpand\@xs@expand@and@detokenize\expandafter\noexpand\@xs@reserved@C}%
				{\let\noexpand\@xs@assign\noexpand\@xs@expand@and@assign\expandafter\noexpand\@xs@reserved@C}}%
		\else
			\def\noexpand#2{\let\noexpand\@xs@assign\noexpand\@xs@expand@and@assign\expandafter\noexpand\@xs@reserved@C}%
		\fi
		\ifx\@empty#3\@empty
		\else
			\def\expandafter\noexpand\@xs@reserved@C{%
				\noexpand\@testopt{\expandafter\noexpand\csname\@xs@reserved@A @@\endcsname}{\ifx\@xs@def\edef#3\else\unexpanded{#3}\fi}}%
		\fi}%
	% Que fait \@xs@reserved@B ? Il d\'efinit :
	% si #3 est vide : \NOM{\@ifstar{\let\@xs@assign\@xs@expand@and@detokenize\@xs@NOM@@}{\let\@xs@assign\@xs@expand@and@assign\@xs@NOM@@}}
	% si #3 existe   : \NOM{\@ifstar{\let\@xs@assign\@xs@expand@and@detokenize\@xs@NOM@}{\let\@xs@assign\@xs@expand@and@assign\@xs@NOM@}}
	%                  \@xs@NOM@{\@testopt{\@xs@NOM@@}{#3}}}
	\@xs@reserved@B
	\ifx\@empty#3\@empty
		\@xs@BuildLines1{#4}{#3}{#1}%
		\@xs@DefArg{#4}%
	\else
		\expandafter\@xs@BuildLines\expandafter1\expandafter{\number\numexpr#4+1}{#3}{#1}%
		\@xs@DefArg@{#4}%
	\fi
	\edef\@xs@reserved@B{\def\expandafter\noexpand\csname\@xs@reserved@A @@\endcsname\@xs@myarg}%
	\edef\@xs@reserved@C{\unexpanded\expandafter{\@xs@newlines}\edef\noexpand\@xs@call}%
	\edef\@xs@reserved@D{\noexpand\noexpand\expandafter\noexpand\csname\@xs@reserved@A\endcsname\unexpanded\expandafter{\@xs@newargs}}%
	\ifnum#5=\@ne\edef\@xs@reserved@D{\noexpand\noexpand\noexpand\@testopt{\unexpanded\expandafter{\@xs@reserved@D}}{}}\fi
	\@xs@edefaddtomacro\@xs@reserved@C{{\unexpanded\expandafter{\@xs@reserved@D}}\noexpand\@xs@call}%
	\@xs@edefaddtomacro\@xs@reserved@B{{\unexpanded\expandafter{\@xs@reserved@C}}}%
	% Que fait \@xs@reserved@B ? Il d\'efinit par exemple pour 3 arguments obligatoires et 1 facultatif :
	%    \def\@xs@NOM@@[##2]##3##4##5{%
	%          \@xs@def\@xs@arg@i{##2}\@xs@assign\@xs@arg@ii{##3}\@xs@assign\@xs@arg@iii{##4}\@xs@asign\@xs@arg@iv{##5}%
	% si #5=0: \edef\@xs@call{\noexpand\@xs@NOM[\@xs@expand\@xs@arg@i]{\@xs@expand\@xs@arg@ii}{\@xs@expand\@xs@arg@iii}{\@xs@expand\@xs@arg@iv}}%
	% si #5=1: \edef\@xs@call{\noexpand\@testopt{\noexpand\@xs@NOM[\@xs@expand\@xs@arg@i]{\@xs@expand\@xs@arg@i}{\@xs@expand\@xs@arg@ii}{\@xs@expand\@xs@arg@iii}{\@xs@expand\@xs@arg@iv}}{}}%
	%          \@xs@call}
	\@xs@reserved@B
	\edef\@xs@reserved@B{\def\expandafter\noexpand\csname\@xs@reserved@A\endcsname\@xs@myarg\ifnum#5=\@ne[\unexpanded{##}\number\numexpr\ifx\@empty#3\@empty#4+1\else#4+2\fi]\fi}%
	% Que fait \@xs@reserved@B ? Il d\'efinit par exemple pour 3 arguments obligatoires et 1 facultatif :
	%    \def \@xs@NOM[##2]##3##4##5[##6]{#6}
	\@xs@reserved@B}

% macro g\'en\'erique qui lit \@xs@reserved@C us par us
% 3 sous-routines sont appel\'ees \`a des moments cl\'e :
% \@xs@atendofgroup      (un groupe se finit, appel r\'ecursif)
% \@xs@atbegingroup      (un groupe vient d'être ouvert)
% \@xs@atnextsyntaxunit  (la future US n'est pas un groupe)
\def\@xs@read@reserved@C{%
	\expandafter\@xs@testempty\expandafter{\@xs@reserved@C}%
	\if@xs@empty
		\ifnum\@xs@nestlevel=\z@
			\let\@xs@next\relax
		\else
			\let\@xs@next\@xs@atendofgroup
		\fi
	\else
		\expandafter\@xs@returnfirstsyntaxunit\expandafter{\@xs@reserved@C}\@xs@reserved@A
		\expandafter\@xs@removefirstsyntaxunit\expandafter{\@xs@reserved@C}\@xs@reserved@C
		\let\@xs@next\@xs@read@reserved@C
		\@xs@exploregroups
		\ifx\bgroup\@xs@toks
			\advance\integerpart\@ne
			\begingroup
				\expandafter\def\expandafter\@xs@reserved@C\@xs@reserved@A
				\@xs@manage@groupID
				\let\@xs@nestlevel\@ne
				\integerpart\z@
				\@xs@atbegingroup
		\else
			\global\advance\decimalpart\@ne
			\@xs@atnextsyntaxunit
		\fi
	\fi
	\@xs@next}

% macro g\'en\'erique qui lit \@xs@reserved@D en proc\'edant \`a des tests avec \IfBeginWith
% 2 sous-routines sont appel\'ees \`a des moments cl\'e :
% \@xs@atendofgroup      (un groupe se finit, appel r\'ecursif)
% \@xs@atoccurfound      (une occurrence a \'et\'e trouv\'ee)
\def\@xs@read@reserved@D{%
	\expandafter\@xs@testempty\expandafter{\@xs@reserved@D}%
	\if@xs@empty
		\ifnum\@xs@nestlevel=\z@
			\let\@xs@next\relax
		\else
			\let\@xs@next\@xs@atendofgroup
		\fi
	\else
		\expandafter\expandafter\expandafter\@xs@IfBeginWith@i\expandafter\expandafter\expandafter{\expandafter\@xs@reserved@D\expandafter}\expandafter{\@xs@reserved@E}%
		{\global\advance\decimalpart\@ne
		 \let\@xs@reserved@D\@xs@reserved@A
		 \@xs@atoccurfound}%
		{\expandafter\@xs@returnfirstsyntaxunit\expandafter{\@xs@reserved@D}\@xs@reserved@A
		 \expandafter\@xs@removefirstsyntaxunit\expandafter{\@xs@reserved@D}\@xs@reserved@D
		 \let\@xs@next\@xs@read@reserved@D
		 \@xs@exploregroups
		 \ifx\bgroup\@xs@toks
		 	\advance\integerpart\@ne
		 	\begingroup
		 		\expandafter\def\expandafter\@xs@reserved@D\@xs@reserved@A
				\@xs@manage@groupID
		 		\let\@xs@reserved@C\@empty
		 		\let\@xs@nestlevel\@ne
		 		\integerpart\z@
		 \else
		 	\expandafter\@xs@addtomacro\expandafter\@xs@reserved@C\expandafter{\@xs@reserved@A}%
		 \fi}%
	\fi
	\@xs@next}

\@xs@newmacro\StrRemoveBraces{}{1}{1}{%
	\def\@xs@reserved@C{#1}%
	\let\@xs@reserved@B\@empty
	\let\@xs@nestlevel\z@
	\@xs@StrRemoveBraces@i
	\expandafter\@xs@ReturnResult\expandafter{\@xs@reserved@B}{#2}}

\def\@xs@StrRemoveBraces@i{%
	\expandafter\@xs@testempty\expandafter{\@xs@reserved@C}%
	\if@xs@empty
		\ifnum\@xs@nestlevel=\z@
			\let\@xs@next\relax
		\else
			\expandafter\endgroup
			\expandafter\@xs@addtomacro\expandafter\@xs@reserved@B\expandafter{\@xs@reserved@B}%
			\let\@xs@next\@xs@StrRemoveBraces@i
		\fi
	\else
		\expandafter\@xs@returnfirstsyntaxunit\expandafter{\@xs@reserved@C}\@xs@reserved@A
		\expandafter\@xs@removefirstsyntaxunit\expandafter{\@xs@reserved@C}\@xs@reserved@C
		\let\@xs@next\@xs@StrRemoveBraces@i
		\ifx\bgroup\@xs@toks
			\ifx\@xs@exploregroups\relax% on explore les groupes ?
				\begingroup
					\expandafter\def\expandafter\@xs@reserved@C\@xs@reserved@A
					\let\@xs@nestlevel\@ne
					\integerpart\z@
					\let\@xs@reserved@B\@empty
			\else
				\expandafter\@xs@addtomacro\expandafter\@xs@reserved@B\@xs@reserved@A
			\fi
		\else
			\expandafter\@xs@addtomacro\expandafter\@xs@reserved@B\expandafter{\@xs@reserved@A}%
		\fi
	\fi
	\@xs@next}

% \@xs@cutafteroccur coupe l'argument #1 apr\`es la #3\`eme occurrence de #2
% \@xs@reserved@C : contient ce qui se trouve avant cette occurrence
% \@xs@reserved@D : contient ce qui se trouve avant cette occurrence y compris cette occurrence
% \@xs@reserved@E : contient ce qui se trouve apr\`es l'occurrence
% si l'occurrence n'existe pas ou qu'un des arguments est vide, toutes les chaines renvoy\'ees sont vides
\def\@xs@cutafteroccur#1#2#3{%
	\def\@xs@reserved@D{#1}\let\@xs@reserved@C\@empty\def\@xs@reserved@E{#2}%
	\decimalpart\z@\integerpart\z@\def\groupID{0}\let\@xs@nestlevel\z@
	\def\@xs@atendofgroup{%
		\expandafter\endgroup
		\expandafter\@xs@addtomacro\expandafter\@xs@reserved@C\expandafter{\expandafter{\@xs@reserved@C}}%
		\@xs@read@reserved@D}%
	\def\@xs@atoccurfound{%
		\ifnum\decimalpart=#3
			\global\let\@xs@reserved@D\@xs@reserved@D
			\global\let\@xs@reserved@C\@xs@reserved@C
			\global\let\groupID\groupID
			\@xs@exitallgroups
			\let\@xs@next\relax
		\else
			\expandafter\@xs@addtomacro\expandafter\@xs@reserved@C\expandafter{\@xs@reserved@E}%
			\let\@xs@next\@xs@read@reserved@D
		\fi}%
	\@xs@read@reserved@D
	\def\@xs@argument@A{#2}%
	\ifnum\decimalpart=#3% occurrence trouv\'ee ?
		\let\@xs@reserved@E\@xs@reserved@D
		\expandafter\expandafter\expandafter\def\expandafter\expandafter\expandafter\@xs@reserved@D\expandafter\expandafter\expandafter{\expandafter\@xs@reserved@C\@xs@argument@A}%
	\else
		\let\@xs@reserved@C\@empty\let\@xs@reserved@E\@empty\let\groupID\@empty
	\fi}

\@xs@newmacro*3\IfSubStr{1}{2}{0}{%
	\def\@xs@argument@A{#2}\def\@xs@argument@B{#3}%
	\expandafter\expandafter\expandafter\@xs@cutafteroccur
	\expandafter\expandafter\expandafter{\expandafter\@xs@argument@A\expandafter}\expandafter{\@xs@argument@B}{#1}%
	\expandafter\@xs@testempty\expandafter{\@xs@reserved@D}%
	\if@xs@empty
		\expandafter\@secondoftwo
	\else
		\expandafter\@firstoftwo
	\fi}

\@xs@newmacro*2\IfBeginWith{}{2}{0}{%
	\def\@xs@argument@A{#1}\def\@xs@argument@B{#2}%
	\expandafter\@xs@testempty\expandafter{\@xs@argument@B}%
	\if@xs@empty
		\let\@xs@next\@secondoftwo
	\else
		\def\@xs@next{\expandafter\expandafter\expandafter\@xs@IfBeginWith@i
			\expandafter\expandafter\expandafter{\expandafter\@xs@argument@A\expandafter}\expandafter{\@xs@argument@B}}%
	\fi
	\@xs@next}

\def\@xs@IfBeginWith@i#1#2{%
	\def\@xs@argument@A{#1}\def\@xs@argument@B{#2}%
	\expandafter\@xs@testempty\expandafter{\@xs@argument@B}%
	\if@xs@empty% #2 est vide, tous les tests sont pass\'es avec succ\`es : on renvoie #3
		\let\@xs@next\@firstoftwo
	\else
		\expandafter\@xs@testempty\expandafter{\@xs@argument@A}%\@xs@testempty{#1}%
		\if@xs@empty
			\let\@xs@next\@secondoftwo% #1 est vide, c'est que #2 est + long que #1 : on renvoie #4
		\else
			\expandafter\@xs@returnfirstsyntaxunit\expandafter{\@xs@argument@A}\@xs@reserved@A
			\expandafter\@xs@returnfirstsyntaxunit\expandafter{\@xs@argument@B}\@xs@reserved@B
			\ifx\@xs@reserved@A\@xs@reserved@B% il y a \'egalit\'e...
				\expandafter\@xs@removefirstsyntaxunit\expandafter{\@xs@argument@A}\@xs@reserved@A% on enl\`eve les 1ere unit\'es syntaxiques
				\expandafter\@xs@removefirstsyntaxunit\expandafter{\@xs@argument@B}\@xs@reserved@B
				\def\@xs@next{% et on recommence avec ces arguments racourcis d'1 unit\'e syntaxique
					\expandafter\expandafter\expandafter\@xs@IfBeginWith@i
					\expandafter\expandafter\expandafter{\expandafter\@xs@reserved@A\expandafter}\expandafter{\@xs@reserved@B}}%
			\else
				\let\@xs@next\@secondoftwo
			\fi
		\fi
	\fi
 	\@xs@next}

\@xs@newmacro*2\IfEndWith{}{2}{0}{%
	\def\@xs@argument@A{#1}\def\@xs@argument@B{#2}%
	\@xs@testempty{#2}%
	\if@xs@empty
		\let\@xs@reserved@A\@secondoftwo
	\else
		\expandafter\expandafter\expandafter\@xs@StrCount
			\expandafter\expandafter\expandafter{\expandafter\@xs@argument@A\expandafter}\expandafter
			{\@xs@argument@B}[\@xs@reserved@A]%
		\ifnum\@xs@reserved@A=\z@
			\let\@xs@reserved@A\@secondoftwo
		\else
			\expandafter\@xs@testempty\expandafter{\@xs@reserved@C}%
			\if@xs@empty
				\let\@xs@reserved@A\@firstoftwo
			\else
				\let\@xs@reserved@A\@secondoftwo
			\fi
		\fi
	\fi
	\@xs@reserved@A}

\@xs@newmacro*4\IfSubStrBefore{1,1}{3}{0}{\@xs@IfSubStrBefore@i[#1]{#2}{#3}{#4}}
\def\@xs@IfSubStrBefore@i[#1,#2]#3#4#5{%
	\def\@xs@reserved@C{#3}%
	\ifx\@xs@exploregroups\relax% si on explore les groupes
		\let\@xs@reserved@B\@empty
		\let\@xs@nestlevel\z@
		\@xs@StrRemoveBraces@i% on retire les accolades
		\let\@xs@reserved@C\@xs@reserved@B
	\fi
	\def\@xs@reserved@A{#5}%
	\expandafter\expandafter\expandafter\@xs@cutafteroccur\expandafter\expandafter\expandafter{\expandafter\@xs@reserved@C\expandafter}\expandafter{\@xs@reserved@A}{#2}%
	\def\@xs@reserved@A{#4}%
	\expandafter\expandafter\expandafter\@xs@cutafteroccur\expandafter\expandafter\expandafter{\expandafter\@xs@reserved@C\expandafter}\expandafter{\@xs@reserved@A}{#1}%
	\let\groupID\@empty
	\expandafter\@xs@testempty\expandafter{\@xs@reserved@C}%
	\if@xs@empty
		\expandafter\@secondoftwo
	\else
		\expandafter\@firstoftwo
	\fi}

\@xs@newmacro*4\IfSubStrBehind{1,1}{3}{0}{\@xs@IfSubStrBehind@i[#1]{#2}{#3}{#4}}
\def\@xs@IfSubStrBehind@i[#1,#2]#3#4#5{\@xs@IfSubStrBefore@i[#2,#1]{#3}{#5}{#4}}

\def\@xs@formatnumber#1#2{%
	\def\@xs@argument@A{#1}%
	\@xs@testempty{#1}%
	\if@xs@empty
		\def#2{0X}% si vide, renvoie 0X
	\else
		\@xs@returnfirstsyntaxunit{#1}\@xs@reserved@A
		\def\@xs@reserved@B{+}%
		\ifx\@xs@reserved@A\@xs@reserved@B
			\expandafter\@xs@removefirstsyntaxunit\expandafter{\@xs@argument@A}\@xs@reserved@C
			\expandafter\@xs@testempty\expandafter{\@xs@reserved@C}%
			\if@xs@empty
			 	\def#2{+0X}%
			 \else
			 	\expandafter\def\expandafter#2\expandafter{\expandafter+\expandafter0\@xs@reserved@C}%
			 \fi
		\else
			\def\@xs@reserved@B{-}%
			\ifx\@xs@reserved@A\@xs@reserved@B
				\expandafter\@xs@removefirstsyntaxunit\expandafter{\@xs@argument@A}\@xs@reserved@A
				\expandafter\@xs@testempty\expandafter{\@xs@reserved@A}%
				\if@xs@empty
				 	\def#2{-0X}%
				 \else
				 	\expandafter\def\expandafter#2\expandafter{\expandafter-\expandafter0\@xs@reserved@A}%
				 \fi
			\else
				\expandafter\def\expandafter#2\expandafter{\expandafter0\@xs@argument@A}%
			\fi
		\fi
	\fi}

\@xs@newmacro\IfInteger{}{1}{0}{%
	\expandafter\@xs@formatnumber\expandafter{\detokenize{#1}}\@xs@reserved@A
	\decimalpart\z@
	\afterassignment\@xs@defafterinteger\integerpart\@xs@reserved@A\relax\@xs@nil
	\expandafter\@xs@testdot\@xs@afterinteger\@xs@nil
	\let\@xs@next\@secondoftwo
	\ifx\@empty\@xs@afterdecimal
		\ifnum\decimalpart=\z@\let\@xs@next\@firstoftwo\fi
	\fi
	\@xs@next}

\@xs@newmacro\IfDecimal{}{1}{0}{%
	\expandafter\@xs@formatnumber\expandafter{\detokenize{#1}}\@xs@reserved@A
	\decimalpart\z@
	\afterassignment\@xs@defafterinteger\integerpart\@xs@reserved@A\relax\@xs@nil
	\expandafter\@xs@testdot\@xs@afterinteger\@xs@nil
	\ifx\@empty\@xs@afterdecimal
		\expandafter\@firstoftwo
	\else
		\expandafter\tokenize\expandafter\@xs@afterdecimal\expandafter{\@xs@afterdecimal}%
		\expandafter\@secondoftwo
	\fi}

\def\@xs@defafterinteger#1\relax\@xs@nil{\def\@xs@afterinteger{#1}}
\def\@xs@testdot{\@ifnextchar.{\@xs@readdecimalpart}{\@xs@testcomma}}
\def\@xs@testcomma{\@ifnextchar,{\@xs@readdecimalpart}{\@xs@endnumber}}
\def\@xs@readdecimalpart#1#2\@xs@nil{%
	\ifx\@empty#2\@empty\def\@xs@reserved@A{0X}\else\def\@xs@reserved@A{0#2}\fi
	\afterassignment\@xs@defafterinteger\decimalpart\@xs@reserved@A\relax\@xs@nil
	\expandafter\@xs@endnumber\@xs@afterinteger\@xs@nil}
\def\@xs@endnumber#1\@xs@nil{\def\@xs@afterdecimal{#1}}

% test d'\'egalit\'e sur des chaines (et des chaines contenant des nombres)
\def\@xs@IfStrEqFalse@i#1#2{\let\@xs@reserved@A\@secondoftwo}
\def\@xs@IfStrEqFalse@ii#1#2{% renvoie vrai si les 2 arg sont d\'ecimaux et s'ils sont \'egaux, faux sinon
	\@xs@IfDecimal{#1}%
		{\@xs@IfDecimal{#2}%
			{\ifdim#1pt=#2pt\let\@xs@reserved@A\@firstoftwo\else\let\@xs@reserved@A\@secondoftwo\fi}% les 2 sont d\'ecimaux : on fait le test
			{\let\@xs@reserved@A\@secondoftwo}}% un seul est d\'ecimal
		{\let\@xs@reserved@A\@secondoftwo}}% #1 n'est pas d\'ecimal

\def\@xs@TestEqual#1#2{% teste si les 2 arguments sont \'egaux
	\def\@xs@reserved@A{#1}\def\@xs@reserved@B{#2}%
	\ifx\@xs@reserved@A\@xs@reserved@B
		\let\@xs@reserved@A\@firstoftwo% \'egalit\'e parfaite des 2 chaines
	\else
		\expandafter\expandafter\expandafter\@xs@reserved@D\expandafter\expandafter\expandafter{\expandafter\@xs@reserved@A\expandafter}\expandafter{\@xs@reserved@B}%
	\fi
	\@xs@reserved@A}

\@xs@newmacro*2\IfStrEq{}{2}{0}{% teste si les deux chaines sont \'egales
	\let\@xs@reserved@D\@xs@IfStrEqFalse@i
	\@xs@TestEqual{#1}{#2}}

\@xs@newmacro*2\IfEq{}{2}{0}{% teste si les 2 arguments (chaine ou nombre) sont \'egaux
	\let\@xs@reserved@D\@xs@IfStrEqFalse@ii
	\@xs@TestEqual{#1}{#2}}

\def\IfStrEqCase{\@ifstar{\def\@xs@reserved@E{\IfStrEq*}\@xs@IfStrCase}{\def\@xs@reserved@E{\IfStrEq}\@xs@IfStrCase}}
\def\@xs@IfStrCase#1#2{\@testopt{\@xs@IfStringCase{#1}{#2}}{}}

\def\IfEqCase{\@ifstar{\def\@xs@reserved@E{\IfEq*}\@xs@IfEqCase}{\def\@xs@reserved@E{\IfEq}\@xs@IfEqCase}}
\def\@xs@IfEqCase#1#2{\@testopt{\@xs@IfStringCase{#1}{#2}}{}}

\def\@xs@IfStringCase#1#2[#3]{%
	\def\@xs@testcase##1##2##3\@xs@nil{% lit les 2 premieres unit\'es syntaxiques dans ##1 et ##2. Les autres dans ##3
		\@xs@reserved@E{#1}{##1}%
			{##2}% le test est positif, on ex\'ecute le code correspondant
			{\@xs@testempty{##3}%
			 \if@xs@empty% le test est n\'egatif
			 	\def\@xs@next{#3}% s'il n'y a plus de cas, on ex\'ecute le code <autres cas>
			 \else
			 	\def\@xs@next{\@xs@testcase##3\@xs@nil}% sinon, on recommence avec ce qui reste
			 \fi
			 \@xs@next}}%
	\@xs@testcase#2\@xs@nil}

% Renvoie ce qui est \`a gauche de l'occurence n°#1 de la sous chaine #3 dans la chaine
\@xs@newmacro*3\StrBefore{1}{2}{1}{%
	\@xs@cutafteroccur{#2}{#3}{#1}%
	\expandafter\@xs@ReturnResult\expandafter{\@xs@reserved@C}{#4}}

% Renvoie ce qui est \`a droite de l'occurence n°#1 de la sous chaine #3 dans la chaine #2
\@xs@newmacro*3\StrBehind{1}{2}{1}{%
	\@xs@cutafteroccur{#2}{#3}{#1}%
	\expandafter\@xs@ReturnResult\expandafter{\@xs@reserved@E}{#4}}

% Renvoie ce qui est strictement compris entre les occurrences n°#1 et n°#2
% des chaines #4 et #5 dans la chaine #3
\@xs@newmacro*4\StrBetween{1,1}{3}{1}{\@xs@StrBetween@i[#1]{#2}{#3}{#4}[#5]}
\def\@xs@StrBetween@i[#1,#2]#3#4#5[#6]{%
	\begingroup
		\noexploregroups
		\@xs@cutafteroccur{#3}{#5}{#2}%
		\expandafter\@xs@cutafteroccur\expandafter{\@xs@reserved@C}{#4}{#1}%
		\expandafter
	\endgroup
	\expandafter\@xs@ReturnResult\expandafter{\@xs@reserved@E}{#6}%
	\let\groupID\@empty}

\def\exploregroups{\let\@xs@exploregroups\relax}
\def\noexploregroups{\def\@xs@exploregroups{\let\@xs@toks0\relax}}
\def\saveexploremode{\let\@xs@saveexploremode\@xs@exploregroups}
\def\restoreexploremode{\let\@xs@exploregroups\@xs@saveexploremode}

% Remplace les #1 premi\`eres occurences de la chaine #3
% par la chaine #4 dans la chaine #2
\@xs@newmacro\StrSubstitute{0}{3}{1}{%
	\def\@xs@reserved@D{#2}\let\@xs@reserved@C\@empty\def\@xs@reserved@E{#3}%
	\def\@xs@argument@C{#3}\def\@xs@argument@D{#4}%
	\decimalpart\z@\integerpart\z@\def\groupID{0}\let\@xs@nestlevel\z@
	\def\@xs@atendofgroup{%
		\expandafter\endgroup
		\expandafter\@xs@addtomacro\expandafter\@xs@reserved@C\expandafter{\expandafter{\@xs@reserved@C}}%
		\@xs@read@reserved@D}%
	\def\@xs@atoccurfound{%
		\ifnum#1<\@ne
			\let\@xs@reserved@A\@xs@argument@D
		\else
			\ifnum\decimalpart>#1
				\let\@xs@reserved@A\@xs@argument@C
			\else
				\let\@xs@reserved@A\@xs@argument@D
			\fi
		\fi
		\expandafter\@xs@addtomacro\expandafter\@xs@reserved@C\expandafter{\@xs@reserved@A}%
		\@xs@read@reserved@D}%
	\@xs@testempty{#3}%
	\if@xs@empty
		\expandafter\@xs@ReturnResult\expandafter{\@xs@reserved@D}{#5}%
	\else
		\@xs@read@reserved@D
		\expandafter\@xs@ReturnResult\expandafter{\@xs@reserved@C}{#5}%
	\fi}

% Supprime les #1 premi\`eres occurrences de #3 dans #2
\@xs@newmacro\StrDel{0}{2}{1}{\@xs@StrSubstitute[#1]{#2}{#3}{}[#4]}

\def\@xs@exitallgroups{\ifnum\@xs@nestlevel>\z@\endgroup\expandafter\@xs@exitallgroups\fi}

% Compte combien d'unit\'es syntaxiques contient la chaine #1 ?
\@xs@newmacro\StrLen{}{1}{1}{%
	\def\@xs@reserved@C{#1}%
	\decimalpart\z@
	\let\@xs@nestlevel\z@
	\def\groupID{0}%
	\let\@xs@atbegingroup\relax
	\def\@xs@atendofgroup{\endgroup\@xs@read@reserved@C}%
	\let\@xs@atnextsyntaxunit\relax
	\@xs@read@reserved@C
	\expandafter\@xs@ReturnResult\expandafter{\number\decimalpart}{#2}}

% Macro interne fermant autant de groupes que n\'ecessaire pour trouver une unit\'e syntaxique derri\`ere
\def\@xs@continuetonext{%
	\expandafter\@xs@testempty\expandafter{\@xs@reserved@C}%
	\if@xs@empty
		\ifnum\@xs@nestlevel>\z@
			\expandafter\endgroup\expandafter\@xs@addtomacro\expandafter\@xs@reserved@B\expandafter{\expandafter{\@xs@reserved@B}}% on concat\`ene
			\expandafter\expandafter\expandafter\@xs@continuetonext% on recommence
		\fi
	\fi}%

\def\@xs@manage@groupID{%
	\begingroup\def\@xs@reserved@A{0}%
	\ifx\@xs@reserved@A\groupID% si on arrive du groupe de niveau 0
		\endgroup\edef\groupID{\number\integerpart}% on met simplement le niveau
	\else
		\endgroup\expandafter\@xs@addtomacro\expandafter\groupID\expandafter{\expandafter,\number\integerpart}%
	\fi}

% Cette macro coupe la chaine #1 apr\`es l'unit\'e syntaxique n°#2
\def\StrSplit{\@ifstar{\let\@xs@reserved@E\@xs@continuetonext\StrSpl@t}{\let\@xs@reserved@E\relax\StrSpl@t}}
\@xs@newmacro\StrSpl@t{}{2}{0}{\@xs@StrSplit@i{#2}{#1}\@xs@StrSplit@ii}
% Cette macro interne coupe la chaine #2 apr\`es l'unit\'e syntaxique n°#1
% Le d\'ebut est assign\'e dans \@xs@reserved@B et la fin dans \@xs@reserved@C
\def\@xs@StrSplit@i#1#2{%
	\def\@xs@reserved@D{#1}\def\@xs@reserved@C{#2}\let\@xs@reserved@B\@empty\let\groupID\@empty
	\ifnum#1>\z@
		\decimalpart\z@\integerpart\z@\def\groupID{0}\let\@xs@nestlevel\z@
		\def\@xs@atendofgroup{%
			\expandafter\endgroup
			\expandafter\@xs@addtomacro\expandafter\@xs@reserved@B\expandafter{\expandafter{\@xs@reserved@B}}%
			\@xs@read@reserved@C}%
		\def\@xs@atbegingroup{\let\@xs@reserved@B\@empty}%
		\def\@xs@atnextsyntaxunit{%
			\expandafter\@xs@addtomacro\expandafter\@xs@reserved@B\expandafter{\@xs@reserved@A}%
			\ifnum\decimalpart=\@xs@reserved@D\relax
				\ifx\@xs@reserved@C\@empty\@xs@reserved@E\fi
				\global\let\@xs@reserved@B\@xs@reserved@B
				\global\let\@xs@reserved@C\@xs@reserved@C
				\global\let\groupID\groupID
				\@xs@exitallgroups
				\let\@xs@next\relax
			\fi}%
		\@xs@read@reserved@C
	\fi}
\def\@xs@StrSplit@ii#1#2{\let#1\@xs@reserved@B\let#2\@xs@reserved@C}

% De la chaine #1, renvoie ce qui se trouve entre les positions
%  #2 et #3, unit\'es syntaxiques aux positions compris !
\@xs@newmacro\StrMid{}{3}{1}{%
	\begingroup
		\noexploregroups
		\let\@xs@reserved@E\relax
		\@xs@StrSplit@i{#3}{#1}%
		\edef\@xs@reserved@C{\number\numexpr#2-1}%
		\let\@xs@reserved@E\relax
		\expandafter\expandafter\expandafter\@xs@StrSplit@i\expandafter\expandafter\expandafter{\expandafter\@xs@reserved@C\expandafter}\expandafter{\@xs@reserved@B}%
	\expandafter\endgroup
	\expandafter\@xs@ReturnResult\expandafter{\@xs@reserved@C}{#4}%
	\let\groupID\@empty}

% supprime #2 unit\'es syntaxiques \`a gauche dans la chaine #1
\@xs@newmacro\StrGobbleLeft{}{2}{1}{%
	\let\@xs@reserved@E\relax
	\@xs@StrSplit@i{#2}{#1}%
	\expandafter\@xs@ReturnResult\expandafter{\@xs@reserved@C}{#3}}

% extrait de #1 la chaine \`a gauche de longueur #2
\@xs@newmacro\StrLeft{}{2}{1}{%
	\let\@xs@reserved@E\relax
	\@xs@StrSplit@i{#2}{#1}%
	\expandafter\@xs@ReturnResult\expandafter{\@xs@reserved@B}{#3}}

% supprime #2 unit\'es syntaxiques \`a droite dans la chaine #1
\@xs@newmacro\StrGobbleRight{}{2}{1}{%
	\@xs@StrLen{#1}[\@xs@reserved@D]%
	\let\@xs@reserved@E\relax
	\expandafter\@xs@StrSplit@i\expandafter{\number\numexpr\@xs@reserved@D-#2}{#1}%
	\expandafter\@xs@ReturnResult\expandafter{\@xs@reserved@B}{#3}}

% renvoie #2 unit\'es syntaxiques \`a la droite de la chaine #1
\@xs@newmacro\StrRight{}{2}{1}{%
	\@xs@StrLen{#1}[\@xs@reserved@D]%
	\let\@xs@reserved@E\relax
	\expandafter\@xs@StrSplit@i\expandafter{\number\numexpr\@xs@reserved@D-#2}{#1}%
	\expandafter\@xs@ReturnResult\expandafter{\@xs@reserved@C}{#3}}

\@xs@newmacro\StrChar{}{2}{1}{%
	\let\@xs@reserved@B\@empty
	\def\@xs@reserved@C{#1}\def\@xs@reserved@D{#2}%
	\ifnum#2>\z@
		\def\groupID{0}\let\@xs@nestlevel\z@\integerpart\z@\decimalpart\z@
		\let\@xs@atbegingroup\relax
		\def\@xs@atendofgroup{\endgroup\@xs@read@reserved@C}%
		\def\@xs@atnextsyntaxunit{%
			\ifnum\decimalpart=\@xs@reserved@D% la n i\`eme US est atteinte ?
				\global\let\@xs@reserved@B\@xs@reserved@A% on capture l'US en cours qui est celle cherch\'ee
				\global\let\groupID\groupID
				\@xs@exitallgroups
				\let\@xs@next\relax
			\fi}%
		\@xs@read@reserved@C
	\fi
	\expandafter\@xs@testempty\expandafter{\@xs@reserved@B}%
	\if@xs@empty\let\groupID\@empty\fi
	\expandafter\@xs@ReturnResult\expandafter{\@xs@reserved@B}{#3}}

% Combien de fois compte t-on #2 dans #1 ?
\@xs@newmacro\StrCount{}{2}{1}{%
	\@xs@testempty{#2}%
	\def\@xs@reserved@D{#1}\def\@xs@reserved@E{#2}\let\@xs@reserved@C\@empty
	\if@xs@empty
		\@xs@ReturnResult{0}{#3}%
	\else
		\decimalpart\z@\integerpart\z@\def\groupID{0}\let\@xs@nestlevel\z@
		\def\@xs@atendofgroup{%
			\expandafter\endgroup
			\expandafter\@xs@addtomacro\expandafter\@xs@reserved@C\expandafter{\expandafter{\@xs@reserved@C}}%
			\@xs@read@reserved@D}%
		\def\@xs@atoccurfound{\let\@xs@reserved@C\@empty\@xs@read@reserved@D}%
		\@xs@read@reserved@D
		\expandafter\@xs@ReturnResult\expandafter{\number\decimalpart}{#3}%
	\fi}

% renvoie la position de l'occurrence #1 de la sous chaine #3 dans la chaine #2
\@xs@newmacro\StrPosition{1}{2}{1}{%
	\@xs@cutafteroccur{#2}{#3}{#1}%
	\let\@xs@reserved@E\groupID
	\ifx\@xs@reserved@C\@xs@reserved@D
		\@xs@ReturnResult{0}{#4}%
		\let\@xs@reserved@E\@empty
	\else
		\expandafter\@xs@StrLen\expandafter{\@xs@reserved@C}[\@xs@reserved@C]%
		\expandafter\@xs@ReturnResult\expandafter{\number\numexpr\@xs@reserved@C+1}{#4}%
	\fi
	\let\groupID\@xs@reserved@E}

\def\comparestrict{\let\@xs@comparecoeff\@ne}
\def\comparenormal{\let\@xs@comparecoeff\z@}
\def\savecomparemode{\let\@xs@saved@comparecoeff\@xs@comparecoeff}
\def\restorecomparemode{\let\@xs@comparecoeff\@xs@saved@comparecoeff}
% Compare les deux arguments #1 et #2
% Renvoie 0 s'ils sont \'egaux et renvoie la
% position de la premiere unit\'e syntaxiques diff\'erente sinon
\@xs@newmacro*2\StrCompare{}{2}{1}{%
	\def\@xs@reserved@A{#1}%
	\def\@xs@reserved@B{#2}%
	\ifx\@xs@reserved@B\@xs@reserved@A
		\@xs@ReturnResult{0}{#3}%
	\else
		\def\@xs@next{\@xs@StrCompare@i{#1}{#2}{#3}}%
		\expandafter\@xs@next
	\fi}

\def\@xs@StrCompare@i#1#2#3{%
	\def\@xs@StrCompare@iii##1{%
		\let\@xs@reserved@A\@empty
		\expandafter\@xs@testempty\expandafter{\@xs@reserved@C}%
		\if@xs@empty
			\def\@xs@reserved@A{*\@xs@comparecoeff}%
		\else
			\expandafter\@xs@testempty\expandafter{\@xs@reserved@D}%
			\if@xs@empty
				\def\@xs@reserved@A{*\@xs@comparecoeff}%
			\fi
		\fi
		\def\@xs@next{%
			\expandafter\@xs@ReturnResult\expandafter
			{\number\numexpr##1\@xs@reserved@A\relax}{#3}}}%
	\def\@xs@StrCompare@ii##1{% ##1 est la position
		\expandafter\@xs@returnfirstsyntaxunit\expandafter{\@xs@reserved@C}\@xs@reserved@A
		\expandafter\@xs@returnfirstsyntaxunit\expandafter{\@xs@reserved@D}\@xs@reserved@B
		\ifx\@xs@reserved@B\@xs@reserved@A
			\expandafter\@xs@testempty\expandafter{\@xs@reserved@A}%
			\if@xs@empty
				\@xs@StrCompare@iii{##1}% les 2 unit\'es syntaxiques sont \'egales, on renvoie la position
			\else
				\def\@xs@next{\expandafter\@xs@StrCompare@ii\expandafter{\number\numexpr##1+1}}% les 2 unit\'es syntaxiques sont \'egales et non vides, on recommence
				\expandafter\@xs@removefirstsyntaxunit\expandafter{\@xs@reserved@C}\@xs@reserved@C
				\expandafter\@xs@removefirstsyntaxunit\expandafter{\@xs@reserved@D}\@xs@reserved@D
			\fi
		\else% les 2 unit\'es syntaxiques sont diff\'erentes : on renvoie la position
			\@xs@StrCompare@iii{##1}%
		\fi
		\@xs@next}%
	\def\@xs@reserved@C{#1}\def\@xs@reserved@D{#2}%
	\@xs@StrCompare@ii1}

\@xs@newmacro\StrFindGroup{}{2}{1}{%
	\def\@xs@reserved@A{#2}\def\@xs@reserved@B{0}%
	\ifx\@xs@reserved@A\@xs@reserved@B
		\def\@xs@next{\@xs@ReturnResult{{#1}}{#3}}%
	\else
		\def\@xs@next{\@xs@StrFindGroup@i{#1}{#2}[#3]}%
	\fi
	\@xs@next}
\def\@xs@StrFindGroup@i#1#2[#3]{%
	\def\@xs@StrFindGroup@ii{%
		\expandafter\@xs@testempty\expandafter{\@xs@reserved@C}%
		\if@xs@empty
			\def\@xs@next{\@xs@ReturnResult{}{#3}}% s'il ne reste plus rien, on renvoie vide
		\else
			\expandafter\@xs@returnfirstsyntaxunit\expandafter{\@xs@reserved@C}\@xs@reserved@D
			\ifx\bgroup\@xs@toks% si la 1\`ere unit\'e syntaxique est un groupe explicite
				\advance\decimalpart\@ne% on augmente le compteur
				\ifnum\decimalpart=\@xs@reserved@A% on est au groupe cherch\'e lors de la profondeur courante ?
					\ifx\@empty\@xs@reserved@B% on est \`a la profondeur maximale ?
						\def\@xs@next{\expandafter\@xs@ReturnResult\expandafter{\@xs@reserved@D}{#3}}% on renvoie ce groupe
					\else% sinon
						\expandafter\def\expandafter\@xs@next\expandafter{\expandafter\@xs@StrFindGroup@i\@xs@reserved@D}% on recommence avec ce groupe
						\expandafter\@xs@addtomacro\expandafter\@xs@next\expandafter{\expandafter{\@xs@reserved@B}[#3]}% et les profondeurs de recherche restantes
					\fi
				\else
					\expandafter\@xs@removefirstsyntaxunit\expandafter{\@xs@reserved@C}\@xs@reserved@C
					\let\@xs@next\@xs@StrFindGroup@ii
				\fi
			\else
				\expandafter\@xs@removefirstsyntaxunit\expandafter{\@xs@reserved@C}\@xs@reserved@C
				\let\@xs@next\@xs@StrFindGroup@ii
			\fi
		\fi
		\@xs@next}%
	\@xs@extractgroupnumber{#2}\@xs@reserved@A\@xs@reserved@B
	\decimalpart\z@
	\ifnum\@xs@reserved@A>\z@\def\@xs@reserved@C{#1}\else\let\@xs@reserved@C\@empty\fi
	\@xs@StrFindGroup@ii}

\def\@xs@extractgroupnumber#1#2#3{%
	\def\@xs@extractgroupnumber@i##1,##2\@xs@nil{\def#2{##1}\def#3{##2}}%
	\@xs@extractgroupnumber@i#1,\@xs@nil
	\ifx\@empty#3\else\@xs@extractgroupnumber@i#1\@xs@nil\fi}

\def\expandingroups{\let\@xs@expandingroups\exploregroups}
\def\noexpandingroups{\let\@xs@expandingroups\noexploregroups}
\def\StrExpand{\@testopt{\@xs@StrExpand}{1}}
\def\@xs@StrExpand[#1]#2#3{%
	\begingroup
		\@xs@expandingroups
		\ifnum#1>\z@
			\integerpart#1\relax
			\decimalpart\z@\def\groupID{0}\let\@xs@nestlevel\z@
			\def\@xs@atendofgroup{%
				\expandafter\endgroup
				\expandafter\@xs@addtomacro\expandafter\@xs@reserved@B\expandafter{\expandafter{\@xs@reserved@B}}%
				\@xs@read@reserved@C}%
			\def\@xs@atbegingroup{\let\@xs@reserved@B\@empty}%
			\def\@xs@atnextsyntaxunit{%
				\expandafter\expandafter\expandafter\@xs@addtomacro
				\expandafter\expandafter\expandafter\@xs@reserved@B
				\expandafter\expandafter\expandafter{\@xs@reserved@A}}%
			\def\@xs@reserved@C{#2}%
			\@xs@StrExpand@i{#1}% Appel de la macro r\'ecursive
		\else
			\def\@xs@reserved@B{#2}%
		\fi
		\global\let\@xs@reserved@B\@xs@reserved@B
	\endgroup
	\let#3\@xs@reserved@B
	\let\groupID\@empty}
\def\@xs@StrExpand@i#1{%
	\ifnum#1>\z@
		\let\@xs@reserved@B\@empty
		\@xs@read@reserved@C
		\let\@xs@reserved@C\@xs@reserved@B
		\def\@xs@reserved@A{\expandafter\@xs@StrExpand@i\expandafter{\number\numexpr#1-1}}%
	\else
		\let\@xs@reserved@A\relax
	\fi
	\@xs@reserved@A}

\def\scancs{\@testopt{\@xs@scancs}{1}}
\def\@xs@scancs[#1]#2#3{%
	\@xs@StrExpand[#1]{#3}{#2}%
	\edef#2{\detokenize\expandafter{#2}}}

% Restaure le code de @
\catcode`\@=\CurrentAtCatcode\relax
% D\'efinit le d\'elimiteur verb
% d\'efinit les diff\'erents modes et les m\'emorise
\setverbdelim{|}%
\fullexpandarg\saveexpandmode
\comparenormal\savecomparemode
\noexploregroups\saveexploremode
\expandingroups
\endinput
%
% Historique
%------------------------------------------------------------------------------
%% v1.0    4/7/2008 : - Package achev\'e.
%          7/7/2008 : - Package publi\'e sur CTAN.
%------------------------------------------------------------------------------
% v1.1    15/8/2008
%   - Le package ne n\'ecessite plus LaTeX et est d\'esormais utilisable sous
%     Plain eTeX.
%   - Ajout des macros \IfInteger et \IfDecimal.
%     Pour cette derni\`ere, la partie enti\`ere et la partie d\'ecimale sont
%     r\'ecup\'erables dans les compteurs \integerpart et \decimalpart. Ce
%     qu'il reste apr\`es qu'un caract\`ere non attendu soit rencontr\'e est
%     dispo dans \@xs@remainafterdecimal
%   - Correction d'un bug dans \tokenize :
%        suppression de l'expansion avec \normalexpandarg pour \'eviter le bug
%        avec les lettres accentu\'ees dans l'exemple : \tokenize\aa{\'e\`u}
%   - Am\'elioration du code de la plupart des macros.
%   - \'Ecriture d'une routine \@xs@newmacro d\'efinissant les  macros.
%   - Suppression de tous les compteurs grace \`a \numexpr.
%   - Nouvelles fonctionnalit\'es internes dans :
%      \IfSubStr
%        ajout des chaines se trouvant avant et apr\`es l'occurrence test\'ee
%        dans les sc \@xs@behind@IfSubStr et \@xs@before@IfSubStr
%      \StrCount
%        a) ajout de ce qui se trouve apr\`es la derni\`ere occurrence dans la
%           sc \@xs@StrCount@afterlastocccur
%        b) la macro ne d\'epend plus d'aucune autre
%------------------------------------------------------------------------------
% v1.2    23/8/2008
%   - Am\'elioration du code de \StrMid \StrGobbleLeft, \StrLeft,
%     \StrGobbleRight et \StrRight \`a l'aide de la nouvelle macro
%     \@xs@StrSplit@i
%   - Nouveau test \IfStrEq qui compare 2 chaines
%   - Nouveau test \IfEq qui compare 2 chaines (ou 2 nombres si les 2 chaines
%     contiennent un nombre)
%   - Correction d'un bug dans \@xs@formatnumber. La macro n'envisageait pas le
%     cas o\`u son argument \'etait vide ce qui faiasait planter
%     \IfDecimal{}{V}{F} et \IfInteger{}{V}{F}
%------------------------------------------------------------------------------
% v1.3    21/9/2008
%  - Am\'elioration du code, mise en place de r\'ecursivit\'es terminales dans
%    toutes les macros r\'ecursives, simplification de \@xs@TestEqual en
%    utilisant \ifx
%  - Nouvelles macros \IfStrEqCase et \IfEqCase
%      Teste si une chaîne est \'egale \`a plusieurs chaînes donn\'ee et
%      ex\'ecute un code sp\'ecifique
%  - Cr\'eation de la macro publique \StrSplit
%      Coupe la chaine en 2 \`a une position donn\'ee
%  - Nouvelle macro \StrCompare
%      Compare 2 chaînes et renvoie la position du 1er caract\`ere diff\'erent.
%      Renvoie 0 si elles sont \'egales.
%------------------------------------------------------------------------------
% v1.3a   29/9/2008
%  - Correction d'un bug : \expandafter#1
%    dans les macros \IfSubStrBefore et \StrBetween qui buggue si #1 est un
%    nombre > 9 !
%  - R\'e \'ecriture de \@xs@returnfirstsyntaxunit et \@gobble qui
%    deviennent purement d\'eveloppables.
%  - R\'e \'ecriture de \StrLen
%  - Nouvelle macro interne \@xs@cutafteroccur
%      Coupe la chaine apr\`es la ni\`eme occurrence d'une sous chaine.
%  - Code am\'elior\'e de \StrMid, \StrLeft, \StrGobbleLeft, \StrRight,
%    \StrGobbleRight grace \`a \@xs@cutafteroccur
%------------------------------------------------------------------------------
% v1.4   4/11/2008
%  - xstring traite ses arguments par unit\'e syntaxique, et donc toutes les
%    macros internes ont \'et\'e r\'e-\'ecrites \`a cette fin.
%  - Le manuel a \'et\'e r\'e-\'ecrit, rendu plus clair et mieux structur\'e.
%  - Nouvelle fonctionnalit\'e : \expandarg
%      le 1er lex\`eme de chaque argument est 1-d\'evelopp\'e avant que la
%      macro ne soit appel\'ee. Si un argument comporte plus qu'1 lex\`eme,
%      il faut passer par \scancs*[1] pour 1-d\'evelopper toutes les unit\'es
%      syntaxiques.
%  - Correction de 2 erreurs dans le manuel anglais :  0 est la valeur par
%    d\'efaut dans \StrSubstitute et \StrDel
%  - Coh\'erence dans les nom des s\'equences de contr\^oles temporaires qui
%    sont d\'esormais : \@xs@reserved@A \`a \@xs@reserved@E
%------------------------------------------------------------------------------
% v1.4a  12/11/2008
%  - Correction d'un bug dans \@xs@StrSplit dans le cas o\`u l'argument
%     num\'erique est <1 : la 1ere coupure doit être vide et le seconde doit
%     être \'egale \`a l'argument.
%------------------------------------------------------------------------------
% v1.4b  16/11/2008
%  - Correction de 2 bugs dans \@xs@returnfirstsyntaxunit
%------------------------------------------------------------------------------
% v1.5   31/12/2008
%  - Nouvelles fonctionnalit\'es dans la recherche de groupes par un
%    identificateur caract\'erisant leur imbrication. Impl\'ementation de :
%      1) \StrFindGroup
%      2) \groupID
%  - Ajout des nouvelles macros g\'en\'eriques \@xs@read@reserved@C et
%    \@xs@read@reserved@D
%  - Correction d'un bug dans \StrSplit : \StrSplit{{a}bc}{1}[\truc] faisait
%    que \truc contenait «a{a}».
%  - Correction d'un bug dans \@xs@newmacro : l'argument optionnel \'etait
%    d\'etok\'enis\'e \`a tort dans les macros \'etoil\'ees.
%  - Dans \@xs@newmacro, on doit choisir le num\'ero du dernier argument devant
%    être d\'etok\'enis\'e dans le cas d'une macro \'etoil\'ee (sachant que
%     l'argument optionnel ne l'est jamais)
%------------------------------------------------------------------------------
% v1.5a  09/2/2009
%  - Nouvelle macro \StrExpand, sensible au mode d'exploration. La macro est
%    indépendante du mode d'exploration et dispose de ses propres commandes
%    d'exploration : \expandingroups et \noexpandingroups
%  - R\'e-\'ecriture de \scancs, qui devient triviale puisque d\'ependant de
%    \StrExpand. Il n'y a plus de version \'étoil\'ee et d\'esormais, \scancs
%    est sensible au mode d'exploration.
%  - Correction d'un bug dans \IfInteger : \IfInteger{2.0}{V}{F} affichait F
%  - Correction de bugs : mettre \let\@xs@reserved@E\relax avant d'appeler
%    \@xs@StrSplit@i
%  - Suppression des messages d'erreur, de warning et d'info. xstring devient
%    donc silencieux ;)
%  - Passage de 3 \'a 2 compteurs
%  - Le manuel est d\'esormais plus color\'e, en esp\'erant qu'il sera un peu
%    plus agr\'eable \`a lire !
%------------------------------------------------------------------------------
% v1.5a  13/3/2009
%  - Modification d'un grand nombre de macros de telle sorte que vraiment
%    n'importe quel code peut d\'esormais \^etre plac\'e dans les arguments des
%    macros (comme par exemple des \if, \ifx ou autre, m\^eme sans leur \fi, ce
%    qui n'\'etait pas possible jusqu'alors)
